Joint Elastic Side-Scattering Lidar and Raman Lidar Measurements of Aerosol Optical Properties in South East Colorado

We describe an experiment, located in south-east Colorado, USA, that measured aerosol optical depth profiles using two Lidar techniques. Two independent detectors measured scattered light from a vertical UV laser beam. One detector, located at the laser site, measured light via the inelastic Raman backscattering process. This is a common method used in atmospheric science for measuring aerosol optical depth profiles. The other detector, located approximately 40km distant, viewed the laser beam from the side. This detector featured a 3.5m2 mirror and measured elastically scattered light in a bistatic Lidar configuration following the method used at the Pierre Auger cosmic ray observatory. The goal of this experiment was to assess and improve methods to measure atmospheric clarity, specifically aerosol optical depth profiles, for cosmic ray UV fluorescence detectors that use the atmosphere as a giant calorimeter. The experiment collected data from September 2010 to July 2011 under varying conditions of aerosol loading. We describe the instruments and techniques and compare the aerosol optical depth profiles measured by the Raman and bistatic Lidar detectors.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
#	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions:

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software.

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE.

# $Id: Makefile,v 1.1 2007-12-17 16:14:43 smueller Exp $

#LATEX = latex
LATEX = pdflatex -shell-escape
BIBTEX = bibtex
MAKEINDEX = makeindex
DVIPDF = dvipdf

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi
RM = rm -f

SRC := $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG = $(SRC:%.tex=%.dvi)
PDF = $(SRC:%.tex=%.pdf)

define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define getpdf
	pdfes=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

#all: $(TRG) $(PDF)
all: $(TRG)

.PHONY: all clean veryclean

clean:
	-rm -f $(TRG) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean: clean
	-rm -fr *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.spl *.ps */*~ *.bak

# This is a rule to generate a file of prerequisites for a given .tex file
%.d: %.tex
	$(get_dependencies) ; echo $$deps;   \
	$(getbibs) ; echo $$bibs ; \
	$(getpdf) ; echo $$epses ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $(wildcard */*.tex) $$bibs $$epses  $(wildcard */*.eps) $$mandeps" > $@

include $(SRC:.tex=.d)

$(TRG): %.dvi : %.tex
	@$(run-latex)

$(PDF): %.pdf : %.dvi
	$(DVIPDF) $<


